Pynsett: A programmable relation extractor

This paper proposes a programmable relation extraction method for the English language by parsing texts into semantic graphs. A person can define rules in plain English that act as matching patterns onto the graph representation. These rules are designed to capture the semantic content of the documents, allowing for flexibility and ad-hoc entities. Relation extraction is a complex task that typically requires sizable training corpora. The method proposed here is ideal for extracting specialized ontologies in a limited collection of documents.

==> acro_list.tex <==
\begin{acronym}[Bi-LSTM]
    \acro{Bi-GCN}{Bi\--directional Graph Convolutional Network}
    \acro{Bi-LSTM}{Bi\--directional Long Short-Term Memory}
    \acro{LSTM}{Long Short-Term Memory}
    \acro{GCN}{Graph Convolutional Network}
    \acro{GRU}{Gated Recurrent Unit}
    \acro{LSTM}{Long Short-Term Memory}
    \acro{NER}{Named Entity Recognition}
    \acro{NLP}{Natural Language Processing}
    \acro{PoS}{Part\--of\--Speech}
    \acro{RNN}{Recurrent Neural Network}
    \acro{EL}{Entity Linking}
    \acro{NED}{Named Entity Disambiguation}
    \acro{WSD}{Word Sense Disambiguation}
\end{acronym}

